Throughput, Bit-Cost, Network State Information: Tradeoffs in Cooperative CSMA Protocols

In wireless local area networks, spatially varying channel conditions result in a severe performance discrepancy between different nodes in the uplink, depending on their position. Both throughput and energy expense are affected. Cooperative protocols were proposed to mitigate these discrepancies. However, additional network state information (NSI) from other nodes is needed to enable cooperation. The aim of this work is to assess how NSI and the degree of cooperation affect throughput and energy expenses. To this end, a CSMA protocol called fairMAC is defined, which allows to adjust the amount of NSI at the nodes and the degree of cooperation among the nodes in a distributed manner. By analyzing the data obtained by Monte Carlo simulations with varying protocol parameters for fairMAC, two fundamental tradeoffs are identified: First, more cooperation leads to higher throughput, but also increases energy expenses. Second, using more than one helper increases throughput and decreases energy expenses, however, more NSI has to be acquired by the nodes in the network. The obtained insights are used to increase the lifetime of a network. While full cooperation shortens the lifetime compared to no cooperation at all, lifetime can be increased by over 25% with partial cooperation.

==> Makefile <==
PROJECT=manni
TMPFILES=*.aux *.bak *.bbl *.blg *.lof *.log *.toc *.lot *~ *.backup\
*.pfx *.ovp $(PROJECT)-pics.* $(PROJECT).dvi $(PROJECT).ps
ARXIVTMP=*.aux *.bak *.blg *.lof *.log *.toc *.lot *~ *.backup\
*.pfx *.ovp $(PROJECT)-pics.* $(PROJECT).dvi $(PROJECT).ps $(PROJECT).pdf *.bib

default: $(PROJECT).tex

clean:
	rm -f $(TMPFILES);
clean_pdf:
	rm -f $(PROJECT).pdf;

$(PROJECT).tex: clean_pdf
	latex $(PROJECT).tex;
	dvips -o $(PROJECT).ps $(PROJECT).dvi;
	ps2pdf14 -sPAPERSIZE=letter -dPDFSETTINGS=/prepress $(PROJECT).ps;

bib:	
	bibtex $(PROJECT);

literatur:
	cp ../references/Literatur.bib ./;
	cp ../references/confs-jrnls.bib ./;
	cp ../references/IEEEabrv.bib ./;
	cp ../references/IEEEtran.cls ./;
	cp ../references/IEEEtran.bst ./;

final: clean clean_pdf
	latex $(PROJECT).tex;
	latex $(PROJECT).tex;
	bibtex $(PROJECT);
	latex $(PROJECT).tex;
	latex $(PROJECT).tex;
	dvips -o $(PROJECT).ps $(PROJECT).dvi;
	ps2pdf14 -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $(PROJECT).ps;
	pdffonts $(PROJECT).pdf;

arxiv:
	rm -f $(ARXIVTMP);
	rm -rf .git;

